Hierarchical Heavy Hitters with the Space Saving Algorithm

The Hierarchical Heavy Hitters problem extends the notion of frequent items to data arranged in a hierarchy. This problem has applications to network traffic monitoring, anomaly detection, and DDoS detection. We present a new streaming approximation algorithm for computing Hierarchical Heavy Hitters that has several advantages over previous algorithms. It improves on the worst-case time and space bounds of earlier algorithms, is conceptually simple and substantially easier to implement, offers improved accuracy guarantees, is easily adopted to a distributed or parallel setting, and can be efficiently implemented in commodity hardware such as ternary content addressable memory (TCAMs). We present experimental results showing that for parameters of primary practical interest, our two-dimensional algorithm is superior to existing algorithms in terms of speed and accuracy, and competitive in terms of space, while our one-dimensional algorithm is also superior in terms of speed and accuracy for a more limited range of parameters.

==> figures.tex <==
\newlength{\figwidth}
\setlength{\figwidth}{0.30\textwidth}
\begin{figure*}
\centering
%1
\subfloat[Memory usage in one dimension. Error bars indicate variation over $N$.]
{
\includegraphics[width=\figwidth]{memory_1000-500_1_33}
\label{figure:memory_1000-500_1_33}
}%
\hspace{0.08in}
\subfloat[Memory usage in two dimensions. Error bars indicate variation over $N$.]
{
\includegraphics[width=\figwidth]{memory_100-50_2}
\label{figure:memory_100-50_2}
}%
%3
\hspace{0.08in}
\subfloat[Memory usage in one dimension for fixed stream length.]
{
\includegraphics[width=\figwidth]{vepsmemory_1}
\label{figure:vepsmemory_1} 
}%
\\
%4
\subfloat[Memory usage in two dimensions for fixed stream length.]
{
\includegraphics[width=\figwidth]{vepsmemory_2}
\label{figure:vepsmemory_2}
}%
%5
\hspace{0.08in}
\subfloat[Speed comparison in two dimensions with high $\epsilon$.]
{
\includegraphics[width=\figwidth]{time_10-5_2}
\label{figure:time_10-5_2}
}%
\hspace{0.08in}
\subfloat[Speed comparison in two dimensions with low $\epsilon$.]
{
\includegraphics[width=\figwidth]{time_1000-500_2}
\label{figure:time_1000-500_2}
}% 
\\
\subfloat[Speed comparison in one dimension with byte-level prefixes and high $\epsilon$.]
{
\includegraphics[width=\figwidth]{time_10-5_1}
\label{figure:time_10-5_1}
}%
\hspace{0.08in}
\subfloat[Speed comparison in one dimension with bit-level prefixes and high $\epsilon$.]
{
\includegraphics[width=\figwidth]{time_10-5_1_33}
\label{figure:time_10-5_1_33}
}%
\hspace{0.08in}
\subfloat[Speed comparison in one dimension with byte-level prefixes and low $\epsilon$.]
{
\includegraphics[width=\figwidth]{time_1000-500_1}
\label{figure:time_1000-500_1}
}%
\\
\subfloat[Speed comparison in one dimension with bit-level prefixes and low $\epsilon$.]
{
\includegraphics[width=\figwidth]{time_1000-500_1_33}
\label{figure:time_1000-500_1_33}
}%
\hspace{0.08in}
\subfloat[Speed comparison in one dimension for fixed stream length.]
{
\includegraphics[width=\figwidth]{vepstime_1}
\label{figure:vepstime_1}
}%
\hspace{0.08in}
\subfloat[Speed comparison in two dimensions for fixed stream length.]
{
\includegraphics[width=\figwidth]{vepstime_2}
\label{figure:vepstime_2}
}%
\caption{Memory and speed comparions.}
\end{figure*}

\begin{figure*}
\subfloat[Output size comparison. Error bars indicate variation over $N$.]
{
\includegraphics[width=\figwidth]{outputsize_100-50_1_33}
\label{figure:outputsize_100-50_1_33}
}%
\hspace{0.08in}
\subfloat[Accuracy comparison in one dimension with byte-level prefixes.]
{
\includegraphics[width=\figwidth]{epsilon_1000-500_1}
\label{figure:epsilon_1000-500_1}
}%
\hspace{0.08in}
\subfloat[Accuracy comparison in two dimensions with byte-level prefixes.]
{
\centering
\includegraphics[width=\figwidth]{epsilon_1000-500_2}
\label{figure:epsilon_1000-500_2}
}%
\caption{Accuracy and output size comparions.}
\end{figure*}
}

